A Reactive Robotized Interface for Lower Limb Rehabilitation: Clinical Results

-This article presents clinical results from the use of MONIMAD, a reactive robotized interface for lower limb Rehabilitation of patients suffering from cerebellar disease. The first problem to be addressed is the postural analysis of sit-to-stand motion. Experiments with healthy subjects were performed for this purpose. Analysis of external forces shows that sit-to-stand transfer can be subdivided into several phases: preaccel-eration, acceleration, start rising, rising. Observation of Center of Pressure, ground forces and horizontal components force on handles yields rules to identify the stability of the patient and to adjust the robotic interface motion to the human voluntary movement. These rules are used in a fuzzy-based controller implementation. The controller is validated on experiments with diseased patients in Bellan Hospital.

==> application.tex <==
The control of the rehabilitation device is designed to help the patient to stand-up.
The design of the fuzzy logic supervisor is based on initial records, the set of data is called ``Data A''.

This first phase is done with an instrumented support handle manipulated by human, recording force and position information and used to help patient to stand-up.  This first set of data, called 'Data A',  is used to identify the robotized of the fuzzy logic supervisor.
This supervisor is then implemented on the robotic device and used to help patients to stand-up.
During these robotic supported experiments data is collected about the action of the supervisor, this set of data is called 'Data B'.

\subsection{Protocol for Data A}



\subsection{Controller tuning}
% Study of the data shows that it is possible to identify each phase of the sit-to-stand motion and also that only force sensors  informations are needed to generate output $\nu_1,\nu_2$ that are represented in figures \ref{fig:set1} and \ref{fig:set2}.


%   \begin{figure}
%  \centering
%  \includegraphics[width=0.45\textwidth,bb=0 0 389 127]{images/fuz_phases_transfert.pdf}
%  % fuz_phases_transfert.pdf: 1179666x1179666 pixel, 300dpi, 9987.84x9987.84 cm, bb=0 0 389 127
%  \caption{Supervisor fuzzy sets of the first output}
%  \label{fig:SupervisorFuzzySet1}
% \end{figure}
%
%
% \begin{figure}
%  \centering
%  \includegraphics[width=0.45\textwidth,bb=0 0 387 149]{force_mem.pdf}
%  % force_mem.pdf: 244x465 pixel, 300dpi, 2.07x3.94 cm, bb=0 0 387 149
%  \caption{Supervisor : fuzzy sets 2nd output}
%  \label{fig:SupervisorFuzzySet2}
% \end{figure}




% \begin{figure}[!hpt]
%  \centering
%  \includegraphics[width=0.49\textwidth]{rec_stab.pdf}
%  % rec_stab.pdf: 1179666x1179666 pixel, 300dpi, 9987.84x9987.84 cm, bb=24 3 492 785
%  \caption{Force during stabilisation and its derivatives}
%  \label{fig:recStab}
% \end{figure}







% \begin{figure}
%  \centering
%  \includegraphics[width=0.48\textwidth,bb=   80   258   514   584]{finalfz_fuz7.pdf}
%  % finalfz_fuz7.pdf: 1179666x1179666 pixel, 300dpi, 9987.84x9987.84 cm, bb=   80   258   514   584
%  \caption{Output of fuzzy supervisor applied on recorded data with Force Handle}
%  \label{fig:FuzModel}
% \end{figure}






